A Domain Semantics for Higher-Order Recursive Processes

The polarized SILL programming language uniformly integrates functional programming and session-typed message-passing concurrency. It supports general recursion, asynchronous and synchronous communication, and higher-order programs that communicate channels and processes. We give polarized SILL a domain-theoretic semantics---the first denotational semantics for a language with this combination of features. Session types in polarized SILL denote pairs of domains of unidirectional communications. Processes denote continuous functions between these domains, and process composition is interpreted by a trace operator. We illustrate our semantics by validating expected program equivalences.

==> conclusion.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

